Abstract Answer Set Solvers with Learning

Nieuwenhuis, Oliveras, and Tinelli (2006) showed how to describe enhancements of the Davis-Putnam-Logemann-Loveland algorithm using transition systems, instead of pseudocode. We design a similar framework for several algorithms that generate answer sets for logic programs: Smodels, Smodels-cc, Asp-Sat with Learning (Cmodels), and a newly designed and implemented algorithm Sup. This approach to describing answer set solvers makes it easier to prove their correctness, to compare them, and to design new systems.

==> smalg.tex <==
We can view
a path in the graph $\sm_\Pi$  as a description of
a process of search for
an answer set for a program $\Pi$ by applying inference
rules.
Therefore, we can characterize the algorithm
of an answer set solver that utilizes the  inference rules of $\sm_\Pi$
 by describing a strategy for choosing a path in 
$\sm_\Pi$. 
A strategy can be based, in particular, on assigning priorities to
some or all inference rules of $\sm_\Pi$, so that a solver will never
apply a transition rule in a state if  a rule with higher priority is applicable
to the same state.

We use this method to describe the {\smodels} 
algorithm. System {\smodels} assigns priorities to the inference rules of 
 $\sm_\Pi$ as follows:
$$
\ba l
\rb,\rf>>\\ 
\ruplp, \rarc, \rbt,\rbf>>\\
\runf>>\\
\rd\hbox{.}
\ea 
$$


For example, let $\Pi$ be program (\ref{ex:pi}).
The {\smodels} algorithm may follow a path
$$
\ba{ll}
\emptyset  &\lrar~(\rd)\\
a^\dec  &\lrar~(\ruplp)\\
a^\dec~c &\lrar~(\rarc)\\
a^\dec~c~\neg b &\lrar~(\runf)\\
a^\dec~c~\neg b~\neg d &\\
\ea
$$ 
in the graph ${\sm}_\Pi$, whereas it may never follow 
path~(\ref{ex:dersuppi}), because {\runf} has a higher priority than {\rd}.


==> supalg.tex <==
In Section~\ref{sec:smalg}  we demonstrated a method 
for specifying the algorithm
of an answer set solver by means of the graph $\sm_\Pi$. 
In particular, we described the {\smodels} algorithm 
by assigning priorities to transition
rules of $\sm_\Pi$. In this section we use this method 
 to describe the {\smodelscc}~\cite{smodelscc} and {\sup}~\cite{lier08} algorithms by means of  $\st_\Pi$.

System {\smodelscc} 
 enhances the {\smodels} algorithm  with conflict-driven backjumping
 and learning. Its strategy for choosing a path in the graph $\st_\Pi$ is
 similar to that of {\smodels}.
 System {\smodelscc} assigns  priorities to  inference
 rules of $\st_\Pi$ as follows:
$$
\ba l
\rbjlp,\rf>>\\ 
\ruplp, \rarc, \rbt,\rbfl>>\\
\runf>>\\
\rd\hbox{.}
\ea 
$$
 
Also, {\smodelscc}  always applies
the transition rule {\rllp}  in a non-semi-terminal  state reached by
an application of {\rbjlp},
because it implements conflict-driven
backjumping and learning.\footnote{ System {\smodelscc} ({\sup}) 
also implements restarts and forgetting that may be modeled by the
transition rules {\rr}
and {\rflp}. An application of these transition rules in
  $\st_\Pi$ relies on particular heuristics implemented by the
solver.}
% This allows modeling conflict-driven
%backjumping and learning implemented by {\smodelscc}. 
In Section~\ref{sec:learn} we discuss  details on which clause is being
learned during the application of {\rllp}.


In~\cite{lier08}, we introduced the simplified {\sup}
 algorithm that relies on backtracking rather than conflict-driven
 backjumping and learning that are actually implemented in the system. We now present the
 {\sup} algorithm that takes these sophisticated techniques into account.

System {\sup} assigns  priorities to  inference
 rules of $\st_\Pi$ as follows:
$$
\ba l
\rbjlp,\rf>>\\ 
\ruplp, \rarc, \rbt,\rbfl>>\\
\rd>>\\
\runf\hbox{.}
\ea 
$$

Similarly to {\smodelscc}, {\sup} always applies
the transition rule {\rllp}  in a non-semi-terminal  state reached by
an application of {\rbjlp}.


For example, let $\Pi$ be program (\ref{ex:pi}). 
Path~(\ref{ex:dersuplpi}) corresponds to an execution of
system {\sup}, but  does not correspond  to any execution 
of {\smodelscc} because for the latter 
{\runf} is a rule of higher priority than {\rd}. Here is another path in
$\st_\Pi$  from $\emptyset||\emptyset$ to the same semi-terminal 
node:
\beq
\ba{ll}
\emptyset||\emptyset  &\lrar~(\rd)\\
a^\dec||\emptyset     &\lrar~(\ruplp)\\
a^\dec~c||\emptyset   &\lrar~(\rarc)\\
a^\dec~c~\neg b||\emptyset &\lrar~(\runf)\\
a^\dec~c~\neg b~\neg d||\emptyset &\\
\ea
\eeq{ex:dersuppi1}
Path~(\ref{ex:dersuppi1}) corresponds to an execution of system
{\smodelscc}, but does not correspond to any execution of system
{\sup} because for the latter 
{\rd} is a rule of higher priority than {\runf}.



The strategy of {\sup} of assigning the transition rule {\runf} the
lowest priority may be reasonable for many problems.  For instance, it is
easy to see that transition rule {\runf} is redundant for
tight programs. The {\sup} algorithm is similar to 
SAT-based answer set solvers such as
{\assat}~\cite{lin04} and
{\cmodels}~\cite{giu06} (see Section~\ref{sec:cmodels}) in the fact
that it will first compute a supported model of a program and only
then will test whether this model is indeed an answer set, i.e.,
whether {\runf} is applicable in this state.



